Optimizing Data Intensive Flows for Networks on Chips

Data flow analysis and optimization is considered for homogeneous rectangular mesh networks. We propose a flow matrix equation which allows a closed-form characterization of the nature of the minimal time solution, speedup and a simple method to determine when and how much load to distribute to processors. We also propose a rigorous mathematical proof about the flow matrix optimal solution existence and that the solution is unique. The methodology introduced here is applicable to many interconnection networks and switching protocols (as an example we examine toroidal networks and hypercube networks in this paper). An important application is improving chip area and chip scalability for networks on chips processing divisible style loads.

==> acknowledgement.tex <==
\section*{Acknowledgments}
“This work has been submitted to the IEEE for possible publication. Copyright may be transferred without notice, after which this version may no longer be accessible.” 

==> append.tex <==
\newpage

\begin{figure*}[htb]
{
\centering
First Name Last Name 1 \\
First Name Last Name 2 \\
\vspace{12pt}
Affiliation \\
Address, City, Country \\
E-mail address
\caption{Example title page heading with 2 authors from the same institution.\label{fig2same}}
}
\end{figure*}

\begin{figure*}[htb]
{
\centering
\begin{tabular}{ccc}
\phantom{Entries to adjust spacing - ignore} & \phantom{intermediate space} & \phantom{Entries to adjust spacing - ignore} \\
First Name Last Name 1 & & First Name Last Name 2 \\
\\
Affiliation 1 & & Affiliation 2 \\
Address, City, Country 1 & & Address, City, Country 2 \\
E-mail address 2 & & E-mail address 2 
\end{tabular}
\caption{Example title page heading with 2 authors from different institutions.\label{fig2different}}
}
\end{figure*}

\begin{figure*}[htb]
{
\centering
\begin{tabular}{ccc}
\phantom{This adjusts spacing - ignore} & \phantom{This adjusts spacing - ignore} & \phantom{This adjusts spacing - ignore} \\
First Name Last Name 1 & & First Name Last Name 2 \\
\\
Affiliation 1 & & Affiliation 2 \\
Address, City, Country 1 & & Address, City, Country 2 \\
E-mail address 1 & & E-mail address 2 \\
\\ \\
& First Name Last Name 3 \\
\\
& Affiliation 3\\
& Address, City, Country 3\\
& E-mail address 3 
\end{tabular}
\caption{Alternate example title page heading with 3 authors from different institutions. \label{fig3different}}
}
\end{figure*}

\begin{figure*}[htb]
{
\centering
\begin{tabular}{ccc}
\phantom{Adjust spacing using these entries} & \phantom{intermediate space} & \phantom{Adjust spacing using these entries} \\
First Name Last Name 1 & & First Name Last Name 2 \\
\\
Affiliation 1 & & Affiliation 2 \\
Address, City, Country 1 & & Address, City, Country 2 \\
E-mail address 1 & & E-mail address 2 \\
\\ \\
First Name Last Name 3 & & First Name Last Name 4 \\
\\
Affiliation 3 & & Affiliation 4 \\
Address, City, Country 3 & & Address, City, Country 4 \\
E-mail address 3 & & E-mail address 4 
\end{tabular}
\caption{Example title page heading with 4 authors from different institutions.\label{fig4different}}
}
\end{figure*}

\begin{figure*}[htb]
{
\centering
\begin{tabular}{ccc}
\phantom{Entries to adjust spacing - ignore} & \phantom{intermediate space} & \phantom{Entries to adjust spacing - ignore} \\
First Name Last Name 1 & & First Name Last Name 3 \\
First Name Last Name 2 & & \\
\\
Affiliation & & Affiliation 3 \\
Address, City, Country & & Address, City, Country 3 \\
E-mail address & & E-mail address 3 
\end{tabular}
\caption{Example title page heading with 3 authors from 2 different institutions. \label{fig2equals1different}}
}
\end{figure*}

==> mesh/RegularMesh_Multi_even.tex <==
\subsection{Multi-source Uniform Data Fraction}
We extend the single source assignment to the multi-source assignment problem  \cite{jia2010scheduling}   \cite{Liu_schedulingdivisible}.  For each processor, we concentrate on the processors' geographical location $P_{i}$, and assigned data fraction $\alpha_{i}$.

Assume the data fractions are distributed uniformly.  For example, the workload is unit $1$ and there are $k$ different data injection options.  So each data injection is assigned $\frac{1}{k}$ workload.

From the data injection position relationship we consider three different situations :
\begin{itemize}
\item Data injection positions consist of a connected subgraph $G_{L}$ of $G$.
\item Data injection processors don't connect with each other.
\item Some data injection positions consist of some connected subgraphs and some are individual injection points.
\end{itemize}


\input{mesh/mesh_multi_even_1.tex}
\input{mesh/mesh_multi_even_2.tex}
\input{mesh/mesh_multi_even_3.tex}
\input{mesh/mesh_multi_even_lowerband.tex}









==> mesh/RegularMesh_SA.tex <==
\subsection{Sensitivity Analysis Virtual Cut-through Switching Scenario}
For a $5*n$ mesh network is in Fig \ref{fig:5t5}, $L$ originate on the inner grid $P_{12}$ and the simulation result says:
\begin{figure}[!ht]
\centering
\includegraphics[width=1\columnwidth]{figure/sa5t5i.eps}
\caption{Sensitivity analysis result of $5*n$ mesh network and the injection position on inner processor $P_{12}$ (where $n = 1 \cdots 5 $)}
\label{fig:sa5t5i}
\end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width=1\columnwidth]{figure/sa5t5i_curve.eps}
\caption{Speedup curves of 5*$n$ mesh network Fig \ref{fig:5t5} (where $n = 1 \cdots 5 $)}
\label{fig:sa5t5i_curve}
\end{figure}
If the number of processor $ > 5$, the cluster equivalence computation ability is at least $5$ time speedup.  There are $5$ processors in the first stage.  For small $\sigma$ speedup growth is linear.  For large $\sigma$ and a large number of cores, speedup is about five as only $P_{0}$ and four adjacent processors do almost all the processing. 



==> mesh/RegularMesh_basic.tex <==
\section{Flow Matrix}
In the virtual cut-through environment, a node can begin relaying the first part of a message (packet) along a transmission path as soon as it starts to arrive at the node , that is, it doesn't have to wait to receive the entire message before it can begin forwarding the message.

First we consider about the $2*2$ mesh network. After, we analyze a more general case $m*n$ mesh network and obtain a general closed-form matrix presentation.  Finally, we give a key methodology to address this type of question. 
\subsection{2*2 Mesh Network}
The load $L$ is assigned on the corner processor $P_{0}$ Fig. ~\ref{fig:2t2}.  The whole task is tackled by four processors $P_{0}$, $P_{1}$, $P_{2}$, $P_{3}$ together.  

\begin{figure}[!ht]
\centering
\includegraphics[width=0.5\columnwidth]{figure/2t2.JPG}
\caption{The 2*2 mesh network and the root processor is $P_{0}$}
\label{fig:2t2}
\end{figure}

The processor $P_{0}$, $P_{1}$ and $P_{2}$ start to process its respective fraction at the same time.  This includes $P_{1}$ and $P_{2}$ as they are relayed load in virtual cut-through mode at $t = 0$.  Because we assume a homogeneous network (in processing speed and communication speed), $\alpha_{1} = \alpha_{2}$ and $P_{1}$ and $P_{2}$ stop processing at the same time.  The processor $P_{3}$ starts to work when the $\alpha_{1}$ and $\alpha_{2}$ complete transmission.  That is, the link $0-1$ and $0-2$ are occupied 
transmitting load to processor $1$ and $2$, respectively and only transmission to $3$ when that is finished.

According to the divisible load theory  \cite{bharadwaj2003divisible}, we obtain the timing diagram Fig. ~\ref{fig:2t2d}.  
\begin{figure}[!ht]
\centering
\includegraphics[width=0.5\columnwidth]{figure/2t2d.JPG}
\caption{The timing diagram for 2*2 mesh network and the root processor is $P_{0}$}
\label{fig:2t2d}
\end{figure}

Here in the Gantt-like timing diagram communication appears above each axis and computations appears below the each axis.  Let's assume that all processors stop computing at the same time in order to minimize the makespan  \cite{sohn1992optimal}.

Based on the timing diagram, we obtain a group of linear equations to find the fraction workload assigned to each processor $\alpha_{i}$ : 

\begin{empheq}[left=\empheqlbrace]
{align}
\alpha_{0} \omega T_{cp} = T_{f, m}\\
\alpha_{1} \omega T_{cp} = T_{f, m}\\
\alpha_{2} \omega T_{cp} = T_{f, m}\\
\alpha_{1}zT_{cm} + \alpha_{3}\omega T_{cp} = T_{f, m}\\
\alpha_{0} + \alpha_{1} + \alpha_{2} + \alpha_{3} = 1\\
\sigma = \frac{zT_{cm}}{\omega T_{cp}}\\
0 < \sigma < 1 \\
0 < \alpha_{0} \leq  1\\
0 \leq  \alpha_{1},  \alpha_{2},  \alpha_{3}  < 1
\end{empheq}
\\

The group of equations are represented by the matrix form:

\begin{equation}
{
\left[ \begin{array}{ccc}
1 & 2 & 1\\
1 & -1 & 0\\
0 & \sigma-1 & 1
\end{array} 
\right ]} \times \left[ \begin{array}{c}
\alpha_{0} \\
\alpha_{1} \\
\alpha_{3} 
\end{array} 
\right ] = \left[ \begin{array}{c}
1 \\
0 \\
0 
\end{array} 
\right ]
\end{equation}
The matrix is represented as $A \times \alpha = b$.  $A$ is named as the \textbf{\textit{flow matrix}}.
Here because of symmetry $\alpha_{1} = \alpha_{2}$, so $\alpha_{2}$ is not listed in the matrix equations.

Finally, the explicit solution is:
\begin{empheq}[left=\empheqlbrace]
{align}
\sigma = \frac{zT_{cm}}{\omega T_{cp}}\\
\alpha_{0} = \frac{1}{4- \sigma}\\
\alpha_{1} = \frac{1}{4- \sigma}\\
\alpha_{3} = \frac{1 - \sigma}{4- \sigma}
\end{empheq}
\\
The simulation result is illustrated:
\begin{figure}[!ht]
\centering
\includegraphics[width=1\columnwidth]{figure/2t2fraction}
\caption{2*2 mesh network.  $\alpha_{0}$, $\alpha_{1}$, $\alpha_{2}$, $\alpha_{3}$ value curve}
\label{fig:2t2fraction}
\end{figure}

In Fig. \ref{fig:2t2fraction},  the three processors $P_{0}$, $P_{1}$, $P_{2}$ three processors have the same data fraction workload, so the curve of $\alpha_{0}$ and $\alpha_{1}$ coincide.  

The figure says that as $\sigma$ grows,  the value $\alpha_{3}$ drops.  In other words, as the communication capacity decreases, there is less data workload assigned to $P_{3}$.  Further, it means it will be economical to keep the load local on $P_{0}$ $P_{1}$ $P_{2}$ and not distribute it, to other processors.  

The equivalence inverse speed of a a single processor is $w_{eq}$, that can replace the original network as
$$\hat{T_{f}} = 1*w_{eq}*T_{cp}$$
$$w_{eq} = \alpha_{0}*w$$
$$Speedup = \frac{T_{f}}{\hat{T_{f}}}= \frac{\omega T_{cp}}{\alpha_{0}\omega T_{cp}} = \frac{1}{\alpha_{0}} = 4- \sigma$$

\subsection{m*n Mesh Network}
Considering a general $m*n$ mesh network,  such as Fig \ref{fig:5t5}. The flow matrix equations for Fig \ref{fig:5t5}:
\begin{equation}
{
\left[ \begin{array}{ccccccccc}
1 & 2 & 3 & 4 & 5 & 4 & 3 & 2 & 1\\
1 & -1 & 0 & 0 & 0 & 0 & 0 & 0& 0\\
0 & \sigma-1 & 1 & 0 & 0 & 0 &0 & 0 & 0 \\
0 & \sigma-1 & \sigma & 1 & 0 & 0 & 0 & 0 & 0 \\
0 & \sigma-1 & \sigma & \sigma & 1 & 0 & 0 & 0 & 0\\
0 & \sigma-1 & \sigma & \sigma & \sigma & 1 & 0& 0 & 0\\
0 & \sigma-1 & \sigma & \sigma & \sigma & \sigma & 1 & 0 & 0\\
0 & \sigma-1 & \sigma & \sigma & \sigma & \sigma & \sigma & 1 & 0\\
0 & \sigma-1 & \sigma & \sigma & \sigma & \sigma & \sigma & \sigma & 1\\
\end{array} 
\right ]} \times \left[ \begin{array}{c}
\alpha_{0} \\
\alpha_{1} \\
\alpha_{3} \\
\alpha_{6} \\
\alpha_{10} \\
\alpha_{15}\\
\alpha_{19}\\
\alpha_{22}\\
\alpha_{24}
\end{array} 
\right ] = \left[ \begin{array}{c}
1 \\
0 \\
0 \\
0 \\
0 \\
0 \\
0 \\
\vdots \\
0
\end{array} 
\right ]
\end{equation}

The proof of $\det A \neq 0$. 
The equivalence inverse processing speed :
$$\hat{T_{f}} = 1*w_{eq}*T_{cp}$$
$$w_{eq} = \alpha_{0}*w$$

so the speedup is:
$$Speedup = \frac{T_{f}}{\hat{T_{f}}}= \frac{\omega T_{cp}}{\alpha_{0}\omega T_{cp}} = \frac{1}{\alpha_{0}} = \left |-\det A \right |$$.

The first row in flow matrix describe the number of cores on each $D_{i}$.  For example, there is 1 core with $0$ hop distance ($D_{0}$) with load site $L$.  There are 2 cores with $1$ hop distance ($D_{1}$) with load site $L$.  There are 3 cores with $2$ hops distance ($D_{2}$) with load site $L$, and so on.  The number of rows means the number of different type processor data fraction.  

  


==> mesh/mesh_multi_even_2_max.tex <==
\subsubsection*{Accelerated Reduced Manhattan Distance Voronoi Diagram Algorithm}
In order to accelerate the bottleneck division computation, we propose a heuristic algorithm to minimize the makespan and give quantitative model analysis utilizing the flow matrix.     

The merits of new algorithm is finishing the task within less makespan as MDVDA and also utilizing less processor resources.
\title{LinearProgram}
\maketitle
\begin{alignat}{2}
\max\quad & Sp_{b}, \label{speedup}\\
\mbox{s.t.}\quad
&\mathop{\sum_{j=0}^{k-1}\sum_{i=0}^{S_{j}-1}} \hat{\alpha_{j,i}} = 1\\
& 1 \geq \hat{\alpha_{j,i}} \geq 0, &{}& \\
& T_{f,i} = \hat{T_{j,f}}, &{i \in 0 \cdots (S_{j}-1)}& \\
&\hat{\alpha_{j,0}}wT_{cp} = \hat{T_{j,f}}, &{j \in 0 \cdots (k-1)}& \\
&\qquad \vdots , &{}&\\
&  (\hat{\alpha_{j,1}} + \cdots \hat{\alpha_{j,l_{j}-2}} )zT_{cm} + \hat{\alpha_{j,l_{j}-1}}wT_{cp} = \hat{T_{j,f}}, &{j \in 0 \cdots (k-1)}& \\
& Sp_{i} = Sp_{b} + \epsilon, &{i \in 0 \cdots (k-1)}& \\
& \epsilon \geq 0 ,&{}&
\end{alignat}
\begin{itemize}
\item Equation \ref{speedup} is the objective function.  Through maximizing the bottleneck cell's speedup, we minimize the makespan. 
\end{itemize}
\newpage
\begin{algorithm}
\caption{Accelerated Reduced Manhattan Distance Voronoi Diagram Algorithm (ARMDVDA)}
\begin{algorithmic} 
\floatname{algorithm}{Procedure}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE  \quad\\
\vspace*{-9pt}
\begin{itemize}
\vspace*{-9pt}
\item $k$ data injection positions
\vspace*{-9pt}
\item $\sigma = \frac{zT_{cm}}{wT_{cp}}$ 
\vspace*{-9pt}
\item processors and links' parameters
\vspace*{-9pt}
\item $f_{T}$ : the requirement of finish time
\vspace*{-9pt}
\item $r_{save}$ : the requirement ratio of saved processors
\vspace*{-9pt}
\item $tmp_{save}$ : the ratio of saved processors
\vspace*{-9pt}
\item $Sp_{i}$ : the speedup of $i$ Voronoi cell.
\vspace*{-9pt}
\item $Sp_{min}$ : $\min  ({Sp_{i}})  \quad i \in 1 \cdots k$
\vspace*{-9pt}
\item $index_{min}$ : the index of $Sp_{min}$
\end{itemize}
	\vspace*{-9pt}
\ENSURE \quad\\
\begin{itemize}
\vspace*{-9pt}
\item $m*n$ processor data fractions $\alpha_{i}$.
\vspace*{-9pt}
\end{itemize}
\vspace*{-5pt}
\STATE Calculate $k$ Voronoi cells with Manhattan distance and $k$ Voronoi cells' radius $R_{i}$.
\STATE Calculate $k$ flow matrix $A_{i}$ and set $depth_{min} = \min ({Sp_{i}})$'s $R_{i}$.
\STATE Calculate the reduced Voronoi cells by setting the $depth_{i} = depth_{min}$ in each Voronoi cell.
\STATE Calculate the determinant of flow matrix.
\STATE Calculate reduced Voronoi cell's flow matrix $\hat{A_{i}}$ and $Sp_{i}$ of each cell.

  		\WHILE{$\frac{1}{Sp_{min}} > f_{T}$ and $tmp_{save} > r_{save}$  }
		\STATE merge processors to $index_{min}$ Voronoi cell one by one
        \STATE by increasing order of $D_{i}$.
		\ENDWHILE

\STATE Calculate $m*n$ processors' data fraction $\alpha_{i}$.
\end{algorithmic}
\end{algorithm}
\newpage

Comparing with RMDVDA, ARMDVDA accelerates the speedup about $20\%$.
\begin{table}[ht]
\caption{The $10$ Accelerated Reduced Voronoi Cells and Speedup Curves}
\centering
\begin{tabular}{c}
\includegraphics[scale=0.63]{figure/voronoi_even_cells_max.eps}\\
\includegraphics[scale=0.63]{figure/voronoi_even_cells_max_speedup.eps}
\end{tabular}
\label{tab:gt_max}
\end{table}

Fig \ref{fig:voronoi_even_cells_max_png} shows the Voronoi cell $3$ is the bottleneck division and there is no other economical way to enlarge this constraint cell.
\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\columnwidth]{figure/voronoi_even_cells_max.png}
\caption{$10$ reduced Voronoi cells}
\label{fig:voronoi_even_cells_max_png}
\end{figure}
\newpage






==> mesh/mesh_multi_even_lowerband.tex <==
\subsubsection{Lower Bound of Intuitive and Heuristic Algorithms}

\begin{itemize}
\item Sp : Speedup of an equivalence computation cell.
\item $optimal_{p}$ : practical optimal speedup of a load data injection, which is NP hard \cite{Liu_schedulingdivisible}.
\item $optimal_{i}$ : optimal speedup of a load data injection in ideal situation
\item $\beta$ :  $\frac{Sp}{optimal_{i}}$ is the ratio between the speedup of an algorithm (i.e. EPSA or RMDVDA) over the practical ideal situation speedup.
\item lower bound : $\beta$ is the value of lower bound.
\end{itemize}

Considering a $n*n$ mesh network, there are $l$ data load injections and the makespan is constrained by the makespan of bottleneck.  So the best solution is that each injection deploys data to its community and the size of community is $\frac{n*n}{l}$.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.5\columnwidth]{figure/max.JPG}
\caption{Maximal speedup for $6*6$ mesh network and $4$ data injections}
\label{fig:max}
\end{figure}


According to the intuitive and heuristic algorithms, we obtain a lower band of these algorithms.

$$\beta = \frac{Sp}{optimal_{i}} \leq \frac{Sp}{optimal_{p}}$$
$$Sp  \geq \beta * optiaml_{p}$$

For example, we calculate a $50*50$ mesh network and there are $l = 10$ load data injections.  Each node transmits data to $\frac{50*50}{10} = 250$ cores.  

In ideal assumption, the first row of flow matrix is $row_{i}$ = [1     4     8    12    16    20    24   28  32  36  40  29];

\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\columnwidth]{figure/maxmesh.JPG}
\caption{Maximal speedup for $16*16$ mesh network and $1$ data injections}
\label{fig:maxmesh}
\end{figure}

We calculate the speedup of a community and the speedup of ideal situation.  In other words, we guarantee obtain a $\beta * optimal_{i}$ times approximation speedup of our algorithms.



==> mesh/reduced_manhattan.tex <==
\subsubsection{Reduced Manhattan Distance Voronoi Diagram Algorithm}
Our objective is to propose a heuristic algorithm to minimize the makespan and give quantitative model analysis utilizing the flow matrix.  The merits of new algorithm is finishing the task within the same makespan as MDVDA, yet utilizing less processor resources.
\title{LinearProgram}
\maketitle
\begin{alignat}{2}
\min\quad & \hat{T_{f}}, \label{objmin}\\
\mbox{s.t.}\quad
&\mathop{\sum_{j=0}^{k-1}\sum_{i=0}^{S_{j}-1}} \hat{\alpha_{j,i}} = 1\\
& 1 \geq \hat{\alpha_{j,i}} \geq 0, &{}& \\
& T_{f,i} = \hat{T_{j,f}}, &{i \in 0 \cdots (S_{j}-1)}& \\
&\hat{\alpha_{j,0}}wT_{cp} = \hat{T_{j,f}}, &{}& \\
&\qquad \vdots , &{}&\\
&  (\hat{\alpha_{j,1}} + \cdots \hat{\alpha_{j,l_{j}-2}})zT_{cm} + \hat{\alpha_{j,l_{j}-1}}wT_{cp} = \hat{T_{j,f}}, &{j \in 0 \cdots (k-1)}& \\
& Sp_{i} = Sp_{b} + \epsilon, &{i \in 0 \cdots (k-1)}& \label{bottom}\\
& \epsilon \geq 0 ,&{}&
\end{alignat}
\begin{itemize}
\item $\hat{T_{f}}$ = $\max{T_{f,i}}, {i \in 0 \cdots (k-1)}$. Equation \ref{objmin} means minimizing the makespan of the whole mesh network.
\item Equation \ref{bottom} means each Voronoi equivalence speedup is approximate same with the bottleneck cell's equivalence speedup.  $\max{T_{f,i}}$ is the speedup of bottleneck cell's finish time.
\item $\epsilon$ is a small enough nonnegative real number.
\end{itemize}

The heuristic algorithm is named as \textbf{\textit{Reduced Manhattan Distance Voronoi Diagram Algorithm}}:
\begin{algorithm}
\caption{Reduced Manhattan Distance Voronoi Diagram Algorithm (RMDVDA)}
\begin{algorithmic} 
\floatname{algorithm}{Procedure}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE $k$ data injection positions
\ENSURE $m*n$ processor data fractions $\alpha_{i}$.
\STATE Calculate $k$ Voronoi cells with Manhattan distance.
\STATE Calculate $k$ Voronoi cells' radius $R_{i}$.
\STATE Calculate $k$ flow matrix $A_{i}$.
\STATE $depth_{min} = \min ({Sp_{i}})$'s $R_{i}$.
\STATE Calculate the reduced Voronoi cells by setting the $depth_{i} = depth_{min}$ in each Voronoi cell.
\STATE Calculate reduced Voronoi cell's flow matrix $\hat{A_{i}}$.
\STATE Calculate $m*n$ processors' data fraction $\alpha_{i}$.
\end{algorithmic}
\end{algorithm}

``Reduced'' means the Voronoi cell shrinks from the outside layer to interior direction layer by layer, which keeps the equivalence computation faster than the bottleneck's computation.  The analysis of the time complexity is the same as EPSA.

\begin{table}[ht]
\caption{The $10$ Reduced Voronoi Cells and speedup curves}
\centering
\begin{tabular}{c}
\includegraphics[scale=0.63]{figure/voronoi_even_cells_save.eps}\\
\includegraphics[scale=0.63]{figure/voronoi_even_speedup_save.eps}
\end{tabular}
\label{tab:gt_reduce}
\end{table}

 Tab \ref{tab:gt_reduce} shows reduced Voronoi cells and reduced Voronoi speedup curves, which saves about $30\%$ processors within the same makespan.

\begin{itemize}
\item Voronoi speedup curves show that $\sigma < 0.2$, the ratio $\max(\frac{Sp_{max}}{Sp_{min}}) = \frac{271}{107} \approx 2.533$.
\item Reduced Voronoi speedup curves show that $\sigma < 0.2$, the ratio is $\max(\frac{Sp_{max}}{Sp_{min}}) = \frac{122}{107} = 1.14$.
\end{itemize}

It displays that $10$ cells' equivalence computation is more balanced than the initial setting, and the whole cluster finishes processing load within the same time by less processors.
After $1000$ round random sampling experiments, we obtain the average saved processors ratio in Fig \ref{fig:voronoi_save}.

\begin{figure}[!ht]
\centering
\includegraphics[width=1\columnwidth]{figure/voronoi_save.eps}
\caption{Reduced Voronoi diagram algorithm average saved processors' percentage}
\label{fig:voronoi_save}
\end{figure}

From the average saved processors ratio Fig \ref{fig:voronoi_save}, it shows the average percentage of saved processor is about $40 \%$.  


